CLIP: Cheap Lipschitz Training of Neural Networks

Despite the large success of deep neural networks (DNN) in recent years, most neural networks still lack mathematical guarantees in terms of stability. For instance, DNNs are vulnerable to small or even imperceptible input perturbations, so called adversarial examples, that can cause false predictions. This instability can have severe consequences in applications which influence the health and safety of humans, e.g., biomedical imaging or autonomous driving. While bounding the Lipschitz constant of a neural network improves stability, most methods rely on restricting the Lipschitz constants of each layer which gives a poor bound for the actual Lipschitz constant. In this paper we investigate a variational regularization method named CLIP for controlling the Lipschitz constant of a neural network, which can easily be integrated into the training procedure. We mathematically analyze the proposed model, in particular discussing the impact of the chosen regularization parameter on the output of the network. Finally, we numerically evaluate our method on both a nonlinear regression problem and the MNIST and Fashion-MNIST classification databases, and compare our results with a weight regularization approach.

==> content/99_Revision.tex <==
\section{Revision}
\begin{enumerate}[label = (R.\Roman*)]
\item  \textcolor{blue}{[Resolved by LB]} The authors are switching from Lip regularization and squared Lip regularization. I think some unification is possible.
\item \textcolor{blue}{[Resolved by LB]} CLIP algorithm is stochastic in nature, however, the analysis is deterministic. Some explanation is required on this issue.
% ---------------------------------------------------------
\item The min-max nature of the considered problem is leveraged to propose CLIP algorithm and is supplemented with good empirical results. However, the theoretical guarantees of CLIP are not provided. At least some discussion on this issue is required.
% ---------------------------------------------------------
\item Using an approximation of Lipschitz constant using a finite subset looses the purpose of the paper and more explanation is required on this issue.
\item \textcolor{blue}{[Resolved by TR]} p.2 "by discussing existence" of solutions ?
% ---------------------------------------------------------
\item \textcolor{blue}{[Resolved by LB]} eq (3): is the choice of the norm linked to the loss function ?
% ---------------------------------------------------------
\item \textcolor{blue}{[Resolved by TR]} p.3 "by a its square"
% ---------------------------------------------------------
\item \textcolor{blue}{[Partially resolved by LB]} p.3 On $X_{Lip}$, I understood the set is fixed from the start. But can it be picked at random at each iteration ? Is there a smart way of detecting the samples for which the Lipschitz constant is probably large ?
\item \textcolor{blue}{[Resolved by LB]} p.6 in proof of Proposition 1, it could be interesting to justify the uniform boundedness of the sequence 
$\theta_i$ to introduce the importance of coercivity discussed later ?
\item \textcolor{blue}{[Resolved by TR]} p.6 in proof of Proposition 1, "don't" to "do not"
% ---------------------------------------------------------
\item \textcolor{blue}{[Resolved by LB]} p.6 Prop 3. What if the realizability condition is not satisfied ? I guess that in case samples are corrupted with noise, can we extend this result to a fitting "up to the level noise" ? Is there any other way to prove the convergence of the sequence $\theta_\lambda$ to $\theta^\dagger$ even without coercivity ? The function can have a local behavior that can be leverage to guarantee it ? I understand it cannot be addressed in this 12-page format, it is just a thought.
% ---------------------------------------------------------
\item \textcolor{blue}{[Resolved by LB]} p.9 Is the network used satisfies the two Assumptions above or it is no intended to be an illustration of them ? The limiting case $\lambda \rightarrow 0$ does not fit the data. Is this behavior linked to realizability assumption not holding or the training step being trapped into a local minima ?
\item p.10 It could be interesting to show how the addition of the Lipschitz regularization increases the computation time of the training process ?
\item The mathematical analysis involves assumption that are, in my opinion, not substantiated enough. I would have appreciated more discussions about the feasibility of them and their validity in the numerical experiment.
\end{enumerate}
